ModelGrow: Continual Text-to-Video Pre-training with Model Expansion and Language Understanding Enhancement

Text-to-video (T2V) generation has gained significant attention recently. However, the costs of training a T2V model from scratch remain persistently high, and there is considerable room for improving the generation performance, especially under limited computation resources. This work explores the continual general pre-training of text-to-video models, enabling the model to "grow" its abilities based on a pre-trained foundation, analogous to how humans acquire new knowledge based on past experiences. There is a lack of extensive study of the continual pre-training techniques in T2V generation. In this work, we take the initial step toward exploring this task systematically and propose ModelGrow. Specifically, we break this task into two key aspects: increasing model capacity and improving semantic understanding. For model capacity, we introduce several novel techniques to expand the model size, enabling it to store new knowledge and improve generation performance. For semantic understanding, we propose a method that leverages large language models as advanced text encoders, integrating them into T2V models to enhance language comprehension and guide generation results according to detailed prompts. This approach enables the model to achieve better semantic alignment, particularly in response to complex user prompts. Extensive experiments demonstrate the effectiveness of our method across various metrics. The source code and the model of ModelGrow will be publicly available.

==> figure/exp_prompt.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{asset/prompt.pdf}
  \caption{We present a comparison between the original prompt and the detailed prompt. Furthermore, we also show the instructions given to the LLaVA-NEXT. The instruction contains the requests for scene specifics, such as setting, lighting, character actions, and camera details, to provide a comprehensive understanding of the video.\todo{Move to supp}}
  \label{fig: prompt}
\end{figure*}

==> figure/main_result_bak.tex <==

\begin{figure*}[htbp]
\captionsetup[subfigure]{labelformat=empty, justification=justified,singlelinecheck=false}
\centering
%
\columnname{Base Model} \hfil
\columnname{Px1} \hfil
\columnname{Px1-LoRA} \hfil
\columnname{Px2} \hfil
\columnname{Px2-LLM}\\
\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/0/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/0/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p_lora/0/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/0/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/0/}{0}{15}
  \caption{Girl with curly hair riding a red bike.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/1/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/1/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p_lora/1/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/1/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/1/}{0}{15}
  \caption{Woman with glasses reading to a little girl.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/2/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/2/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p_lora/2/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/2/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/2/}{0}{15}
  \caption{Pink motorcycle weaving through orange traffic cones.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/3/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/3/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p_lora/3/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/3/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/3/}{0}{15}
  \caption{Dancer with metallic skin twirling near a glowing tree.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/4/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/4/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p_lora/4/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/4/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/4/}{0}{15}
  \caption{Pig with wings flying above a diamond mountain.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  %\caption{Girl with curly hair riding a red bike.}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/5/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p/5/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/stage4/5/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2/5/}{0}{15}
  \animategraphics[controls=none, width=0.18\textwidth]{8}{asset/figure5/lc_p2_llm_sl/5/}{0}{15}
  \caption{Crystal chandelier swinging above a wooden table.}
  % \put(-470,36){Input Image}
\end{subfigure}%

\caption{Our results compared with baselines. Viewing the video with Adobe Acrobat.}
\label{fig: main_examples}
\end{figure*}

==> figure/mehtod_block_expansion.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{asset/block_expansion.pdf}
  \caption{The vanilla transformer blocks and three model expansion variants.}
  \label{fig: dit}
\end{figure*}

==> figure/teaser_backup.tex <==
% \begin{figure*}[t]
%   \centering
%   %\includegraphics[width=\linewidth]{asset/exp1.gif}
%   %\includemovie{10cm}{10cm}{asset/exp1.gif}
%   \animategraphics[controls, width=0.4\textwidth]{8}{asset/teaser/0/}{0}{15}
%    \animategraphics[controls, width=0.4\textwidth]{8}{asset/teaser/1/}{0}{15}
%     \animategraphics[controls, width=0.4\textwidth]{8}{asset/teaser/2/}{0}{15}
%     \animategraphics[controls, width=0.4\textwidth]{8}{asset/teaser/3/}{0}{15}
%   \caption{We continue to pre-train a text-to-video diffusion model with block duplicated expansion and language understanding enhancement via LLMs. We show examples frame by frame. We generate videos with high quality, semantics consistency, and diverse motion, given a long, detailed prompt.}
%   \label{fig: teaser}
% \end{figure*}


\begin{figure*}[htbp]
\captionsetup[subfigure]{labelformat=empty, justification=justified,singlelinecheck=false}
\centering
%
\begin{subfigure}{\textwidth}
  \centering
  \caption{Pikachu snowboarding.}
  %\animategraphics[controls, width=0.23\textwidth]{8}{asset/teaser/0/}{0}{15}
  % \includegraphics[width=0.25\linewidth]{asset/teaser/0/0.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/0/5.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/0/10.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/0/15.png}
  \vrule \hspace{0.5pt}
  \animategraphics[controls=none, width=0.23\textwidth]{8}{asset/teaser/0/}{0}{15}
  % \put(-470,36){Input Image}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
    \caption{  A stack of pancakes is drizzled with syrup, the golden liquid flowing over the edges.}
  %\animategraphics[controls, width=0.23\textwidth]{8}{asset/teaser/1/}{0}{15}
  % \includegraphics[width=0.25\linewidth]{asset/teaser/1/0.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/1/5.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/1/10.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/1/15.png}
  \vrule \hspace{0.5pt}
  \animategraphics[controls=none, width=0.23\textwidth]{8}{asset/teaser/1/}{0}{15}
\end{subfigure}% 

\begin{subfigure}{\textwidth}
  \centering
  \caption{An astronaut flying in space.}
  %\animategraphics[controls, width=0.23\textwidth]{8}{asset/teaser/2/}{0}{15}
  % \includegraphics[width=0.25\linewidth]{asset/teaser/0/0.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/2/5.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/2/10.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/2/15.png}
  \vrule \hspace{0.5pt}
  \animategraphics[controls=none, width=0.23\textwidth]{8}{asset/teaser/2/}{0}{15}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
  \caption{Blue apple bouncing near a pink tree.}
  %\animategraphics[controls, width=0.23\textwidth]{8}{asset/teaser/3/}{0}{15}
  % \includegraphics[width=0.25\linewidth]{asset/teaser/3/0.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/3/5.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/3/10.png}
  \includegraphics[width=0.23\linewidth]{asset/teaser/3/15.png}
  \vrule \hspace{0.5pt}
  \animategraphics[controls=none, width=0.23\textwidth]{8}{asset/teaser/3/}{0}{15}
\end{subfigure}%
\caption{We continue to pre-train a text-to-video diffusion model with \textbf{model expansion} and \textbf{language understanding enhancement via LLMs}. We show three frames of each example, and \textbf{the video on the last column is better viewed with Adobe Acrobat}. We generate videos with high quality, semantics consistency, and diverse motion, given a general prompt.}
\end{figure*}

==> figure/teaser_backup_1113.tex <==
\twocolumn[{
\maketitle
\begin{center}
    \captionsetup{type=figure}
% \begin{figure*}[htbp]
% \captionsetup[subfigure]{labelformat=empty, justification=justified,singlelinecheck=false}
% \centering
%
\begin{tabular}{c@{}@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}}
    \centering
    \put(20,0){Pikachu snowboarding.}
    \put(190,0){\textbf{Click me}}
    \put(240,10){Pancakes drizzled with syrup,}
    \put(240,0){the golden liquid flowing over the edges.}
    \put(420,0){\textbf{Click me}}
    &&&&&&& \\
    \rotatebox{90}{Base} &
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/3/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/3/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/3/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/stage4/3/}{0}{15}&
    % case 2
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/0/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/0/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/0/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/stage4/0/}{0}{15}\\

    \rotatebox{90}{Ours}\hspace{2pt} & 
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/0/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/0/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/0/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/lc_p2_llm/0/}{0}{15}&
    % case 2
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/1/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/1/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/1/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/lc_p2_llm/1/}{0}{15}\\
    % case3
    \put(20,0){An astronaut flying in space.}
    \put(240,0){Blue apple bouncing near a pink tree.}
    %\put(260,70){the golden liquid flowing over the edges.}
    &&&&&&& \\
    \rotatebox{90}{Base}\hspace{2pt} &
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/2/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/2/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/2/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/stage4/2/}{0}{15}&
    % case 4
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/1/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/1/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/stage4/1/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/stage4/1/}{0}{15}\\

    \rotatebox{90}{Ours}\hspace{2pt} &
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/2/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/2/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/2/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/lc_p2_llm/2/}{0}{15}&
    % case 4
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/3/5.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/3/10.png}\hspace{-2pt}&
    \includegraphics[width=0.11\linewidth]{asset/teaser/lc_p2_llm/3/15.png}&
    \vrule \hspace{0.5pt}
    \animategraphics[controls=none, width=0.11\textwidth]{8}{asset/teaser/lc_p2_llm/3/}{0}{15}\\
\end{tabular}

\captionof{figure}{We continue to pre-train a text-to-video diffusion model with model expansion and language understanding enhancement via LLMs. We show three frames of each example, and \textbf{the video below ``Click me'' is better viewed with Adobe Acrobat}. We generate videos with high quality, semantics consistency, and diverse motion, given a general prompt.}
%\end{figure*}
\end{center}
}]

==> figure/teaser_label.tex <==
\twocolumn[{
\maketitle

\begin{figure*}
    \includegraphics[width=1\linewidth]{asset/teaser/label_v1.pdf}
\end{figure*}

}]
